Material Recognition in the Wild with the Materials in Context Database

Recognizing materials in real-world images is a challenging task. Real-world materials have rich surface texture, geometry, lighting conditions, and clutter, which combine to make the problem particularly difficult. In this paper, we introduce a new, large-scale, open dataset of materials in the wild, the Materials in Context Database (MINC), and combine this dataset with deep learning to achieve material recognition and segmentation of images in the wild. MINC is an order of magnitude larger than previous material databases, while being more diverse and well-sampled across its 23 categories. Using MINC, we train convolutional neural networks (CNNs) for two tasks: classifying materials from patches, and simultaneous material recognition and segmentation in full images. For patch-based classification on MINC we found that the best performing CNN architectures can achieve 85.2% mean class accuracy. We convert these trained CNN classifiers into an efficient fully convolutional framework combined with a fully connected conditional random field (CRF) to predict the material at every pixel in an image, achieving 73.1% mean class accuracy. Our experiments demonstrate that having a large, well-sampled dataset such as MINC is crucial for real-world material recognition and segmentation.

==> raw_scores.tex <==
Point Test Cls & Point Test Tot & Pixel Test Cls & Pixel Test Tot & Ensemble & Ensemble Op & Aggregation ID \\
\textbf{85.0\%} & \textbf{84.5\%} & 64.2\% & 73.3\% & 1, 7, 8 & sum & 7 \\
\textbf{84.9\%} & \textbf{84.9\%} & 64.3\% & 74.1\% & 1, 7, 8 & prod & 7 \\
\textbf{84.6\%} & \textbf{84.1\%} & 62.9\% & 71.2\% & 1, 2, 7 & sum & 7 \\
\textbf{84.6\%} & \textbf{84.6\%} & 64.1\% & 73.2\% & 1, 2, 3, 7 & prod & 7 \\
\textbf{84.6\%} & \textbf{84.3\%} & 64.4\% & 73.1\% & 1, 2, 3, 7 & sum & 7 \\
\textbf{84.5\%} & \textbf{84.2\%} & 62.6\% & 71.1\% & 1, 2, 7 & prod & 7 \\
\textbf{84.4\%} & \textbf{84.1\%} & 64.6\% & 73.6\% & 1, 2, 3, 7, 8, 18 & sum & 7 \\
\textbf{84.2\%} & 83.0\% & 61.0\% & 69.0\% & 1, 7, 18 & sum & 7 \\
\textbf{84.2\%} & \textbf{84.2\%} & 64.9\% & 74.1\% & 1, 2, 3, 7, 8 & sum & 7 \\
\textbf{84.2\%} & \textbf{84.5\%} & 64.8\% & 74.5\% & 1, 2, 3, 7, 8 & prod & 7 \\
84.0\% & \textbf{84.3\%} & 64.5\% & 74.0\% & 1, 2, 3, 7, 8, 18 & prod & 7 \\
83.9\% & 82.8\% & 60.3\% & 68.1\% & 1, 7 & sum & 7 \\
83.8\% & 83.6\% & 64.5\% & 73.6\% & 1 & sum & 30 \\
83.8\% & 83.6\% & 64.5\% & 73.5\% & 54 & sum & 30 \\
83.8\% & 82.9\% & 60.6\% & 69.0\% & 1, 7, 18 & prod & 7 \\
83.8\% & 83.6\% & 64.5\% & 73.5\% & 54 & sum & 39 \\
83.7\% & 83.6\% & 64.5\% & 73.6\% & 54 & sum & 32 \\
83.7\% & 83.5\% & 63.8\% & 72.7\% & 1 & sum & 28 \\
83.7\% & 83.6\% & 64.6\% & 73.6\% & 1 & sum & 32 \\
83.7\% & 83.5\% & 64.5\% & 73.6\% & 1 & sum & 25 \\
83.7\% & 83.4\% & 64.1\% & 73.0\% & 1 & sum & 34 \\
83.7\% & 83.5\% & 64.4\% & 73.5\% & 54 & sum & 25 \\
83.7\% & 83.5\% & 64.3\% & 73.5\% & 1 & sum & 31 \\
83.7\% & 83.6\% & 65.1\% & 74.5\% & 1 & sum & 26 \\
83.6\% & 83.6\% & 64.5\% & 73.6\% & 1 & sum & 39 \\
83.6\% & 83.4\% & 64.2\% & 73.5\% & 1 & sum & 29 \\
83.6\% & 83.4\% & 63.7\% & 72.6\% & 54 & sum & 28 \\
83.6\% & 83.3\% & 64.1\% & 72.9\% & 54 & sum & 34 \\
83.5\% & 83.6\% & 64.2\% & 73.5\% & 54 & sum & 33 \\
83.5\% & 83.6\% & 64.3\% & 73.6\% & 1 & sum & 33 \\
83.5\% & 83.5\% & 65.1\% & 74.4\% & 54 & sum & 26 \\
83.5\% & 82.9\% & 61.6\% & 69.9\% & 64 & sum & 7 \\
83.5\% & 83.1\% & 62.8\% & 71.5\% & 54 & sum & 24 \\
83.5\% & 83.4\% & 64.3\% & 73.4\% & 54 & sum & 31 \\
83.5\% & 83.2\% & 62.9\% & 71.6\% & 1 & sum & 24 \\
83.5\% & 82.6\% & 59.6\% & 67.9\% & 1, 7 & prod & 7 \\
83.5\% & 83.5\% & 65.6\% & 75.2\% & 1 & sum & 27 \\
83.5\% & 83.2\% & 63.5\% & 72.3\% & 1, 3, 18 & sum & 7 \\
83.4\% & 83.1\% & 62.5\% & 71.2\% & 1, 2, 18 & prod & 7 \\
83.4\% & 82.7\% & 61.2\% & 69.5\% & 71 & sum & 7 \\
83.4\% & 83.5\% & 65.6\% & 75.1\% & 54 & sum & 27 \\
83.4\% & 83.2\% & 63.0\% & 71.6\% & 1, 2 & sum & 7 \\
83.3\% & 83.3\% & 64.2\% & 73.4\% & 54 & sum & 29 \\
83.3\% & 83.1\% & 62.6\% & 71.1\% & 1, 2, 18 & sum & 7 \\
83.3\% & 83.2\% & 63.0\% & 71.7\% & 1, 2 & prod & 7 \\
83.2\% & 82.8\% & 61.6\% & 69.8\% & 63 & sum & 7 \\
83.2\% & 83.2\% & 63.3\% & 72.4\% & 1, 3, 18 & prod & 7 \\
83.2\% & 82.4\% & 60.9\% & 69.1\% & 58 & sum & 7 \\
83.2\% & 82.4\% & 60.9\% & 69.1\% & 59 & sum & 7 \\
83.2\% & 82.4\% & 60.9\% & 69.1\% & 61 & sum & 7 \\
83.2\% & 82.7\% & 61.4\% & 69.6\% & 70 & sum & 7 \\
83.2\% & 83.3\% & 64.1\% & 73.1\% & 1, 2, 3 & sum & 7 \\
83.1\% & 82.5\% & 61.1\% & 69.4\% & 1 & sum & 7 \\
83.1\% & 82.5\% & 61.1\% & 69.4\% & 67 & sum & 7 \\
83.1\% & 83.3\% & 64.5\% & 73.8\% & 1, 2, 8 & sum & 7 \\
83.1\% & 83.1\% & 64.1\% & 73.1\% & 1, 3 & sum & 7 \\
83.1\% & 82.4\% & 61.0\% & 69.3\% & 54 & sum & 7 \\
83.1\% & 82.4\% & 61.0\% & 69.3\% & 60 & sum & 7 \\
83.1\% & 82.3\% & 60.9\% & 69.1\% & 57 & sum & 7 \\
83.1\% & 82.3\% & 60.9\% & 69.1\% & 68 & sum & 7 \\
83.1\% & 82.3\% & 60.9\% & 69.1\% & 69 & sum & 7 \\
83.0\% & 82.3\% & 61.2\% & 69.5\% & 1, 18 & prod & 7 \\
82.9\% & 82.3\% & 61.2\% & 69.4\% & 1, 18 & sum & 7 \\
82.9\% & 83.2\% & 64.0\% & 73.2\% & 1, 2, 3 & prod & 7 \\
82.8\% & 83.1\% & 63.9\% & 73.3\% & 1, 3 & prod & 7 \\
82.8\% & 83.2\% & 64.4\% & 74.1\% & 1, 2, 8 & prod & 7 \\
82.8\% & 82.8\% & 64.2\% & 73.7\% & 1, 8 & sum & 7 \\
82.3\% & 82.7\% & 64.2\% & 74.1\% & 1, 8 & prod & 7 \\
82.3\% & 82.2\% & 62.7\% & 71.5\% & 2 & sum & 7 \\
82.2\% & 82.4\% & \textbf{66.7\%} & 76.5\% & 54 & sum & 38 \\
82.2\% & 82.3\% & 64.2\% & 73.7\% & 1, 3, 8 & sum & 7 \\
82.0\% & 82.3\% & \textbf{66.7\%} & 76.5\% & 1 & sum & 38 \\
81.9\% & 82.3\% & 63.9\% & 73.9\% & 1, 3, 8 & prod & 7 \\
81.8\% & 81.1\% & 60.4\% & 67.7\% & 62 & sum & 7 \\
81.2\% & 80.7\% & 59.1\% & 67.2\% & 55 & sum & 7 \\
80.9\% & 80.5\% & 58.8\% & 67.0\% & 56 & sum & 7 \\
80.5\% & 79.9\% & 58.3\% & 66.3\% & 18 & sum & 7 \\
79.4\% & 80.2\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 43 \\
79.3\% & 80.1\% & \textbf{66.5\%} & 76.7\% & 1 & sum & 43 \\
79.0\% & 79.5\% & 61.5\% & 71.7\% & 3 & sum & 7 \\
78.7\% & 79.7\% & \textbf{66.8\%} & 76.8\% & 54 & sum & 54 \\
78.5\% & 79.6\% & 65.7\% & 76.0\% & 56 & sum & 41 \\
78.5\% & 79.6\% & \textbf{66.8\%} & 76.8\% & 54 & sum & 55 \\
78.4\% & 79.7\% & 66.0\% & 76.3\% & 62 & sum & 41 \\
78.3\% & 79.3\% & 65.8\% & 76.1\% & 55 & sum & 41 \\
78.2\% & 76.2\% & 51.7\% & 57.8\% & 7 & sum & 7 \\
78.2\% & 79.3\% & \textbf{66.8\%} & 76.8\% & 54 & sum & 56 \\
78.0\% & 79.2\% & \textbf{66.7\%} & 76.8\% & 54 & sum & 57 \\
78.0\% & 79.5\% & \textbf{66.3\%} & 76.0\% & 1, 7 & prod & 41 \\
78.0\% & 79.1\% & \textbf{66.2\%} & 76.6\% & 70 & sum & 41 \\
77.9\% & 79.1\% & \textbf{66.4\%} & 76.7\% & 71 & sum & 41 \\
77.8\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 58 & sum & 41 \\
77.8\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 59 & sum & 41 \\
77.8\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 61 & sum & 41 \\
77.8\% & 79.0\% & \textbf{66.3\%} & 76.7\% & 63 & sum & 41 \\
77.7\% & 78.9\% & \textbf{66.5\%} & 76.7\% & 54 & sum & 41 \\
77.7\% & 78.9\% & \textbf{66.5\%} & 76.7\% & 60 & sum & 41 \\
77.7\% & 79.3\% & \textbf{67.1\%} & 77.4\% & 1, 2, 7 & prod & 41 \\
77.7\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 57 & sum & 41 \\
77.7\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 68 & sum & 41 \\
77.7\% & 78.9\% & \textbf{66.5\%} & 76.6\% & 69 & sum & 41 \\
77.6\% & 78.9\% & \textbf{66.3\%} & 76.7\% & 64 & sum & 41 \\
77.6\% & 78.9\% & \textbf{66.4\%} & 76.0\% & 1, 7 & sum & 41 \\
77.5\% & 78.7\% & \textbf{66.3\%} & 76.6\% & 1 & sum & 41 \\
77.5\% & 78.7\% & \textbf{66.3\%} & 76.6\% & 67 & sum & 41 \\
77.4\% & 78.8\% & 65.7\% & 76.1\% & 56 & sum & 44 \\
77.3\% & 78.7\% & 65.8\% & 75.9\% & 1, 7, 18 & prod & 41 \\
77.3\% & 78.9\% & 65.9\% & 76.3\% & 62 & sum & 44 \\
77.0\% & 78.5\% & 65.9\% & 76.3\% & 55 & sum & 44 \\
76.7\% & 78.1\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 46 \\
76.7\% & 78.1\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 58 \\
76.6\% & 78.6\% & \textbf{67.2\%} & \textbf{78.1\%} & 1, 2, 3, 7 & prod & 41 \\
76.6\% & 78.0\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 47 \\
76.6\% & 77.9\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 59 \\
76.6\% & 78.3\% & \textbf{67.0\%} & 77.1\% & 1, 2, 7 & sum & 41 \\
76.5\% & 78.3\% & 65.9\% & 75.8\% & 1, 7 & prod & 44 \\
76.5\% & 77.0\% & 60.1\% & 69.7\% & 7 & sum & 41 \\
76.4\% & 77.9\% & 65.7\% & 75.7\% & 1, 7, 18 & sum & 41 \\
76.4\% & 77.9\% & \textbf{66.6\%} & 76.5\% & 58 & sum & 44 \\
76.4\% & 77.9\% & \textbf{66.6\%} & 76.5\% & 59 & sum & 44 \\
76.4\% & 77.9\% & \textbf{66.6\%} & 76.5\% & 61 & sum & 44 \\
76.4\% & 78.0\% & 65.9\% & 76.6\% & 70 & sum & 44 \\
76.4\% & 77.8\% & \textbf{66.6\%} & 76.7\% & 54 & sum & 44 \\
76.4\% & 77.8\% & \textbf{66.6\%} & 76.7\% & 60 & sum & 44 \\
76.3\% & 78.0\% & \textbf{66.2\%} & 76.6\% & 71 & sum & 44 \\
76.3\% & 77.8\% & 65.5\% & 75.9\% & 1, 18 & prod & 41 \\
76.3\% & 77.8\% & 65.9\% & 76.5\% & 63 & sum & 44 \\
76.3\% & 77.7\% & \textbf{66.5\%} & 76.6\% & 54 & sum & 48 \\
76.2\% & 77.7\% & \textbf{66.5\%} & 76.7\% & 54 & sum & 60 \\
76.2\% & 77.8\% & \textbf{66.5\%} & 76.6\% & 57 & sum & 44 \\
76.2\% & 77.8\% & \textbf{66.5\%} & 76.6\% & 68 & sum & 44 \\
76.2\% & 77.8\% & \textbf{66.5\%} & 76.6\% & 69 & sum & 44 \\
76.2\% & 77.7\% & \textbf{66.3\%} & 76.6\% & 54 & sum & 42 \\
76.1\% & 78.1\% & \textbf{66.3\%} & 77.3\% & 1, 2 & prod & 41 \\
76.1\% & 78.1\% & \textbf{66.7\%} & 77.2\% & 1, 2, 7 & prod & 44 \\
76.1\% & 77.8\% & 66.0\% & 76.6\% & 64 & sum & 44 \\
76.0\% & 77.5\% & \textbf{66.5\%} & 76.6\% & 54 & sum & 49 \\
76.0\% & 77.6\% & 66.1\% & 75.9\% & 1, 7 & sum & 44 \\
76.0\% & 77.5\% & \textbf{66.5\%} & 76.6\% & 54 & sum & 61 \\
76.0\% & 77.5\% & 65.5\% & 75.8\% & 1, 18 & sum & 41 \\
76.0\% & 77.4\% & 65.5\% & 75.8\% & 1, 7, 18 & prod & 44 \\
75.9\% & 78.1\% & \textbf{66.6\%} & \textbf{78.3\%} & 1, 7, 8 & prod & 41 \\
75.9\% & 77.6\% & \textbf{66.2\%} & 76.6\% & 1 & sum & 44 \\
75.9\% & 77.6\% & \textbf{66.2\%} & 76.6\% & 67 & sum & 44 \\
75.9\% & 77.8\% & \textbf{66.3\%} & 76.9\% & 1, 2, 18 & prod & 41 \\
75.9\% & 77.4\% & \textbf{66.4\%} & 76.7\% & 54 & sum & 62 \\
75.7\% & 77.5\% & 66.1\% & 76.5\% & 1 & sum & 42 \\
75.7\% & 77.3\% & \textbf{66.4\%} & 76.6\% & 54 & sum & 63 \\
75.6\% & 77.8\% & \textbf{66.2\%} & 77.2\% & 1, 2 & sum & 41 \\
75.4\% & 77.4\% & \textbf{66.2\%} & 76.8\% & 1, 2, 18 & sum & 41 \\
75.4\% & 76.9\% & \textbf{66.3\%} & 76.6\% & 54 & sum & 64 \\
75.1\% & 76.8\% & \textbf{66.3\%} & 76.6\% & 54 & sum & 65 \\
74.9\% & 77.2\% & \textbf{66.7\%} & \textbf{78.0\%} & 1, 2, 3, 7 & prod & 44 \\
74.9\% & 76.9\% & \textbf{66.7\%} & 76.9\% & 1, 2, 7 & sum & 44 \\
74.9\% & 77.4\% & \textbf{66.7\%} & \textbf{78.3\%} & 1, 2, 3, 7, 8, 18 & prod & 41 \\
74.9\% & 77.2\% & 65.9\% & 77.3\% & 1, 3, 18 & prod & 41 \\
74.8\% & 76.5\% & 65.4\% & 75.8\% & 1, 18 & prod & 44 \\
74.8\% & 77.4\% & \textbf{66.8\%} & \textbf{78.5\%} & 1, 2, 3, 7, 8 & prod & 41 \\
74.8\% & 77.2\% & \textbf{66.8\%} & \textbf{78.0\%} & 1, 2, 3, 7 & sum & 41 \\
74.7\% & 76.6\% & 66.1\% & 76.5\% & 54 & sum & 37 \\
74.6\% & 76.4\% & 65.3\% & 75.5\% & 1, 7, 18 & sum & 44 \\
74.6\% & 75.7\% & 59.8\% & 69.9\% & 7 & sum & 44 \\
74.6\% & 77.1\% & \textbf{66.5\%} & \textbf{78.0\%} & 1, 2, 3 & prod & 41 \\
74.6\% & 76.9\% & 65.9\% & 77.2\% & 1, 2 & prod & 44 \\
74.6\% & 77.1\% & \textbf{66.7\%} & \textbf{78.1\%} & 1, 3 & prod & 41 \\
74.4\% & 76.1\% & 65.2\% & 75.7\% & 1, 18 & sum & 44 \\
74.3\% & 76.6\% & 66.0\% & 76.9\% & 1, 2, 18 & prod & 44 \\
74.3\% & 76.4\% & 65.8\% & 76.4\% & 1 & sum & 37 \\
74.1\% & 76.5\% & 65.8\% & 77.1\% & 1, 2 & sum & 44 \\
74.1\% & 75.5\% & 63.4\% & 73.3\% & 18 & sum & 41 \\
74.1\% & 76.7\% & 65.8\% & 77.0\% & 2 & sum & 41 \\
74.1\% & 76.7\% & \textbf{66.2\%} & \textbf{78.1\%} & 1, 7, 8 & prod & 44 \\
73.9\% & 74.6\% & 58.4\% & 69.7\% & 8 & sum & 7 \\
73.8\% & 76.2\% & 65.8\% & 77.0\% & 1, 3, 18 & sum & 41 \\
73.8\% & 76.4\% & \textbf{66.4\%} & \textbf{77.8\%} & 1, 2, 3 & sum & 41 \\
73.7\% & 75.9\% & 65.9\% & 76.6\% & 1, 2, 18 & sum & 44 \\
73.5\% & 76.1\% & \textbf{66.3\%} & \textbf{77.7\%} & 1, 3 & sum & 41 \\
73.4\% & 76.3\% & \textbf{66.3\%} & \textbf{78.1\%} & 1, 2, 8 & prod & 41 \\
73.4\% & 76.1\% & \textbf{66.3\%} & \textbf{78.3\%} & 1, 2, 3, 7, 8, 18 & prod & 44 \\
73.3\% & 75.9\% & 65.6\% & 77.2\% & 1, 3, 18 & prod & 44 \\
73.3\% & 75.9\% & \textbf{66.3\%} & \textbf{78.0\%} & 1, 7, 8 & sum & 41 \\
73.2\% & 75.9\% & \textbf{66.3\%} & \textbf{78.0\%} & 1, 2, 3, 7, 8, 18 & sum & 41 \\
73.1\% & 75.9\% & \textbf{66.4\%} & \textbf{78.0\%} & 1, 3 & prod & 44 \\
73.1\% & 75.7\% & \textbf{66.4\%} & \textbf{77.9\%} & 1, 2, 3, 7 & sum & 44 \\
73.1\% & 75.9\% & 66.1\% & \textbf{78.0\%} & 1, 2, 3 & prod & 44 \\
73.1\% & 76.1\% & \textbf{66.4\%} & \textbf{78.4\%} & 1, 2, 3, 7, 8 & prod & 44 \\
73.0\% & 75.7\% & \textbf{66.5\%} & \textbf{78.1\%} & 1, 2, 3, 7, 8 & sum & 41 \\
72.8\% & 75.5\% & 65.5\% & 77.0\% & 2 & sum & 44 \\
72.6\% & 75.7\% & 65.8\% & \textbf{77.8\%} & 1, 8 & prod & 41 \\
72.5\% & 74.3\% & 63.2\% & 73.2\% & 18 & sum & 44 \\
72.3\% & 75.1\% & 66.0\% & \textbf{77.8\%} & 1, 2, 8 & sum & 41 \\
72.2\% & 74.8\% & 65.5\% & 76.9\% & 1, 3, 18 & sum & 44 \\
72.2\% & 75.1\% & 66.1\% & \textbf{77.7\%} & 1, 2, 3 & sum & 44 \\
72.0\% & 74.8\% & 66.0\% & \textbf{77.6\%} & 1, 3 & sum & 44 \\
71.9\% & 75.1\% & 66.0\% & \textbf{78.0\%} & 1, 2, 8 & prod & 44 \\
71.9\% & 75.1\% & 65.6\% & 77.4\% & 1, 3, 8 & prod & 41 \\
71.5\% & 74.4\% & 66.0\% & \textbf{77.9\%} & 1, 2, 3, 7, 8, 18 & sum & 44 \\
71.3\% & 74.3\% & 65.9\% & \textbf{77.8\%} & 1, 7, 8 & sum & 44 \\
71.2\% & 74.2\% & 65.4\% & 77.4\% & 1, 8 & sum & 41 \\
71.2\% & 74.2\% & 66.1\% & \textbf{78.0\%} & 1, 2, 3, 7, 8 & sum & 44 \\
71.2\% & 74.5\% & 65.6\% & \textbf{77.7\%} & 1, 8 & prod & 44 \\
70.9\% & 73.9\% & 65.3\% & 77.1\% & 1, 3, 8 & sum & 41 \\
70.7\% & 73.5\% & 65.4\% & 76.1\% & 54 & sum & 36 \\
70.6\% & 73.7\% & 65.5\% & \textbf{77.7\%} & 1, 2, 8 & sum & 44 \\
70.5\% & 73.9\% & 65.3\% & 77.3\% & 1, 3, 8 & prod & 44 \\
70.4\% & 73.3\% & 65.1\% & 76.0\% & 1 & sum & 36 \\
70.2\% & 73.2\% & 64.0\% & 76.0\% & 3 & sum & 41 \\
69.5\% & 72.7\% & 65.0\% & 77.1\% & 1, 8 & sum & 44 \\
69.3\% & 72.6\% & 65.0\% & 77.0\% & 1, 3, 8 & sum & 44 \\
68.8\% & 71.9\% & 64.1\% & 76.1\% & 3 & sum & 44 \\
64.9\% & 68.3\% & 60.7\% & 73.5\% & 8 & sum & 41 \\
64.7\% & 69.0\% & 62.2\% & 73.5\% & 54 & sum & 50 \\
64.6\% & 68.9\% & 62.2\% & 73.5\% & 54 & sum & 51 \\
64.5\% & 68.8\% & 62.2\% & 73.5\% & 54 & sum & 52 \\
64.4\% & 68.8\% & 62.2\% & 73.5\% & 54 & sum & 53 \\
63.5\% & 67.1\% & 60.3\% & 73.4\% & 8 & sum & 44 \\




\hline CNN & Min dim. & \# shifts & \# scales & Scale range & Mirror \\ \hline
1 & 1100 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
2 & 800 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
3 & 550 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
7 & 2200 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
8 & 386 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
18 & 1100 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
54 & 1100 & 1 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
55 & 1100 & 2 & 1 & 1 & N \\
56 & 1100 & 1 & 1 & 1 & N \\
57 & 1100 & 2 & 5 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
58 & 1100 & 1 & 5 & $[1/\sqrt{2}, \sqrt{2}]$ & N \\
59 & 1100 & 1 & 5 & $[1/2, 2]$ & N \\
60 & 1100 & 1 & 3 & $[1/2, 2]$ & N \\
61 & 1100 & 1 & 5 & $[1/3, 3]$ & N \\
62 & 1100 & 1 & 1 & 1 & Y \\
63 & 1100 & 1 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & Y \\
64 & 1100 & 2 & 3 & $[1/\sqrt{2}, \sqrt{2}]$ & Y \\
67 & 1100 & 2 & 3 & $[1/2, 2]$ & N \\
68 & 1100 & 2 & 5 & $[1/2, 2]$ & N \\
69 & 1100 & 2 & 5 & $[1/3, 3]$ & N \\
70 & 1100 & 1 & 5 & $[1/\sqrt{2}, \sqrt{2}]$ & Y \\
71 & 1100 & 2 & 7 & $[1/\sqrt{2}, \sqrt{2}]$ & Y \\




\hline CRF & $w_p$  & $\theta_p$ & $\theta_L$ & $\theta_{ab}$ \\ \hline
7 & 0 & N/A & N/A & N/A \\
24 & 1.000 & 0.200 & 20.000 & 5.000 \\
25 & 2.000 & 0.200 & 20.000 & 5.000 \\
26 & 2.500 & 0.200 & 20.000 & 5.000 \\
27 & 3.000 & 0.200 & 20.000 & 5.000 \\
28 & 1.500 & 0.200 & 20.000 & 5.000 \\
29 & 2.000 & 0.200 & 20.000 & 10.000 \\
30 & 2.000 & 0.200 & 20.000 & 2.500 \\
31 & 2.000 & 0.200 & 40.000 & 5.000 \\
32 & 2.000 & 0.200 & 10.000 & 5.000 \\
33 & 2.000 & 0.400 & 20.000 & 5.000 \\
34 & 2.000 & 0.100 & 20.000 & 5.000 \\
36 & 13.606 & 0.189 & 15.365 & 4.726 \\
37 & 10.000 & 0.189 & 15.365 & 4.726 \\
38 & 5.000 & 0.189 & 15.365 & 4.726 \\
39 & 2.000 & 0.189 & 15.365 & 4.726 \\
41 & 8.000 & 0.189 & 15.365 & 4.726 \\
42 & 9.000 & 0.189 & 15.365 & 4.726 \\
43 & 7.000 & 0.189 & 15.365 & 4.726 \\
44 & 8.000 & 0.189 & 15.365 & 4.726 \\
46 & 7.800 & 0.189 & 15.365 & 4.726 \\
47 & 7.900 & 0.189 & 15.365 & 4.726 \\
48 & 8.100 & 0.189 & 15.365 & 4.726 \\
49 & 8.200 & 0.189 & 15.365 & 4.726 \\
50 & 7.800 & 0.189 & 15.365 & 4.726 \\
51 & 7.900 & 0.189 & 15.365 & 4.726 \\
52 & 8.100 & 0.189 & 15.365 & 4.726 \\
53 & 8.200 & 0.189 & 15.365 & 4.726 \\
54 & 7.800 & 0.189 & 15.365 & 4.726 \\
55 & 7.900 & 0.189 & 15.365 & 4.726 \\
56 & 8.100 & 0.189 & 15.365 & 4.726 \\
57 & 8.200 & 0.189 & 15.365 & 4.726 \\
58 & 7.800 & 0.189 & 15.365 & 4.726 \\
59 & 7.900 & 0.189 & 15.365 & 4.726 \\
60 & 8.100 & 0.189 & 15.365 & 4.726 \\
61 & 8.200 & 0.189 & 15.365 & 4.726 \\
62 & 7.800 & 0.200 & 20.000 & 5.000 \\
63 & 7.900 & 0.200 & 20.000 & 5.000 \\
64 & 8.100 & 0.200 & 20.000 & 5.000 \\
65 & 8.200 & 0.200 & 20.000 & 5.000 \\

